Pseudorandomness via the discrete Fourier transform

We present a new approach to constructing unconditional pseudorandom generators against classes of functions that involve computing a linear function of the inputs. We give an explicit construction of a pseudorandom generator that fools the discrete Fourier transforms of linear functions with seed-length that is nearly logarithmic (up to polyloglog factors) in the input size and the desired error parameter. Our result gives a single pseudorandom generator that fools several important classes of tests computable in logspace that have been considered in the literature, including halfspaces (over general domains), modular tests and combinatorial shapes. For all these classes, our generator is the first that achieves near logarithmic seed-length in both the input length and the error parameter. Getting such a seed-length is a natural challenge in its own right, which needs to be overcome in order to derandomize RL - a central question in complexity theory. Our construction combines ideas from a large body of prior work, ranging from a classical construction of [NN93] to the recent gradually increasing independence paradigm of [KMN11, CRSW13, GMRTV12], while also introducing some novel analytic machinery which might find other applications.

==> Fourier.tex <==
% !TEX root = main.tex
\section{Reduction to fooling Fourier transforms}
\ignore{
In this section we construct generator to fool linear threshold functions to polynomial
error with seedlength $\tilde{O}(\log n)$ proving Theorem
\ref{th:mainintrohs}. As the generator and its analysis is quite
technical, we first give a high-level description.

For simplicity, in this discussion let us fix a test vector $v \in
\R^n$ and error $\epsilon = 1/\poly(n)$.
}

Define the Kolomogorov distance between two integer values random
variables $Z_1, Z_2$ as
\begin{align}
\label{eq:cdf-dist}
 d_K(Z_1,Z_2) = \max_{k \in \mathbb{Z}}(|\pr(Z_1\leq k) - \pr(Z_2\leq
k)|).
\end{align}

The starting point of our analysis and construction is to note that
showing closeness in Kolmogorov for discrete random variables of
relatively small support is equivalent to showing that the
\emph{Fourier transforms} of the random variables are close. This will
allow us to use various analytic tools. Concretely, we shall use the
following elementary fact about the discrete Fourier transform.

\begin{lem}\label{lem:introfouriertocdf}
Let $Z_1, Z_2$ be two integer valued random variables supported on $[-N,N]$. Then,
\[ d_K(Z_1,Z_2) \leq O(\log(N)) \cdot \max_{\alpha \in [0,1]}
\left|\E[\exp(2\pi i \alpha Z_1)] - \E[\exp(2\pi i \alpha
  Z_2)]\right|.\]
\end{lem}
\begin{proof}
By definition we have that
$$
d_K(Z_1,Z_2) = \max_{-N\leq k \leq N}(|\pr(Z_1\leq k) - \pr(Z_2\leq k)|).
$$
Suppose that
$$
\delta = \max_{\alpha \in [0,1]} \left|\E[\exp(2\pi i \alpha Z_1)] - \E[\exp(2\pi i \alpha Z_2)]\right|.
$$
We note that
\begin{align*}
\pr(Z_i\leq k) & = \sum_{j=-N}^k \pr(Z_i=j)\\
& = \sum_{j=-N}^k \int_0^1 \exp(-2\pi i j \alpha) \E[\exp(2\pi i \alpha Z_i)] d\alpha\\
& = \int_0^1 s(k,N,\alpha)\E[\exp(2\pi i \alpha Z_i)] d\alpha
\end{align*}
where
\[ s(k,N,\alpha) = \sum_{j=-N}^k  \exp(-2\pi i j \alpha) .\]
It is clear that $|s(k,N,\alpha)| \leq 2N$. Further,
\begin{align*} |s(k,N,\alpha)| & = \left|\frac{\exp(-2\pi i k\alpha)
  (\exp(2\pi i (N+k+1)\alpha)-1)}{\exp(2\pi i \alpha)-1}\right|  \leq \frac{1}{|\exp(2\pi i \alpha)
    -1|} \leq O(\frac{1}{[\alpha]})
\end{align*}
where $[\alpha]$ is the distance between $\alpha$ and the nearest integer.
Therefore, we have
\begin{align*}
|\pr(Z_1\leq k) - \pr(Z_2\leq k)|  & \leq \int_0^1 |s(k,N,\alpha)|\left|\E[\exp(2\pi i \alpha Z_1)]-\E[\exp(2\pi i \alpha Z_1)] \right|d\alpha \\
& \leq \int_0^1 O\left(\min\left(N,\frac{1}{[\alpha]}\right)\right)\delta d\alpha\\
& = O(\delta) \left(\int_0^{1/N} Nd\alpha + \int_{1/N}^{1/2}\frac{d\alpha}{\alpha} + \int_{1/2}^{1-1/N} \frac{d\alpha}{1-\alpha} + \int_{1-1/N}^1 N d\alpha\right)\\
& = O(\delta \log(N)).
\end{align*}

\end{proof}
%The above implies the following corollary with regards to fooling linear threshold functions.
As a corollary we get the following regarding fooling linear threshold functions.
\ignore{\begin{cor}\label{LTFtoFTCor}
Suppose that $X$ and $Y$ are two random variables supported on $\{\pm 1\}^n$. Suppose furthermore that for every $v\in \R^n$ that
$$
\left|\E[\phi_v(X)] - \E[\phi_v(Y)]\right| \leq \delta,
$$
then for any linear threshold function, $f$ we have that
$$
\left|\E[f(X)]-\E[f(Y)] \right| = O(\delta n \log(n)).
$$
\end{cor}}
\begin{cor}\label{LTFtoFTCor}
Let $X, Y$ be two random variables supported on $\dpm^n$ such that for all $v \in \R^n$,
$$
\left|\E[\phi_v(X)] - \E[\phi_v(Y)]\right| \leq \delta.
$$
Then for any linear threshold function, $f:\dpm^n \to \dpm$, we have
$$
\left|\E[f(X)]-\E[f(Y)] \right| = O(\delta n \log(n)).
$$
\end{cor}
\begin{proof}
We may write $f(x)=\sgn(v\cdot x+\theta)$ for $v\in \Z^n$ with coordinates of absolute value at most $n^{O(n)}$, and $\theta\in\Z$ of absolute value at most $n^{O(n)}$. Letting $Z_1=v\cdot X+\theta$ and $Z_2=v\cdot Y+\theta$, then $Z_1,Z_2$ are both integer-valued random variables with range contained in $[-N,N]$ for $N\leq n^{O(n)}$. Furthermore,
$$
\left|\E[f(X)]-\E[f(Y)] \right| = 2\left|\pr(Z_1<0)-\pr(Z_2<0) \right| \leq 2 d_K(Z_1,Z_2).
$$
We may thus apply Lemma \ref{lem:introfouriertotv} to obtain
$$
\left|\E[f(X)]-\E[f(Y)] \right| = O\left(n\log(n)\max_{\alpha\in\R}\left|\E[\exp(2\pi i \alpha Z_1)] - \E[\exp(2\pi i \alpha Z_2)]\right| \right).
$$
We note that for any given $\alpha$
\begin{align*}
\left|\E[\exp(2\pi i \alpha Z_1)] - \E[\exp(2\pi i \alpha Z_2)]\right| & = \left|\exp(2\pi i \alpha\theta)\left(\E[\exp(2\pi i \alpha (v\cdot X))]-\E[\exp(2\pi i \alpha (v\cdot Y))] \right) \right|\\
& = \left|\E[\phi_{\alpha v}(X)] - \E[\phi_{\alpha v}(Y)] \right|\\
& \leq \delta.
\end{align*}
This completes the proof.
\end{proof}

It is well known that fooling halfspaces with polynomially small error
requires fooling all modular tests where the modulus $m \leq
\poly(n)$. We give a simple argument in Appendix \ref{app:modular}
directly showing that fooling the
Fourier transform suffices to fool all modular tests.

We now show that it suffices to consider $\phi_v$ for $v$ such that $|v_i| \leq 1/4$
where each $v_i$ can be represented using bounded precision.

\begin{lem}
\label{lem:bounded}
Suppose that $X$ and $Y$ are random variables supported on $\{\pm 1\}^n$ such that
\[ \left|\E[\phi_v(X)] - \E[\phi_v(Y)]\right| \leq \delta \]
holds for $v$ such that for every $i \in [n]$,
\begin{itemize}
\item $v_i\in [-1/4,1/4]$.
\item $v_i$ can be represented with $O(\log(n/\delta))$ bits of precision.
\end{itemize}
Then for all $v \in \R^n$,
\[ \left|\E[\phi_v(X)] - \E[\phi_v(Y)]\right| \leq O(\delta). \]
\end{lem}
\begin{proof}
Since $\phi_v(x) = \exp(2\pi i \sum_i v_ix_i)$, by shifting each $v_i$
by an integer, it suffices to consider $v_i \in [-1/2,1/2]$. Further,
for every $v \in [-1/2,1/2]^n$, we claim there exists $v' \in
[-1/4,1/4]^n$ and $b \in \{-1,1\}$ such that for all $x \in \pmo^n$,
$\phi_v(x) = b\phi_{v'}(x)$, hence
\[
\left|\E[\phi_v(X)] - \E[\phi_v(Y)]\right|  = \left|\E[b\phi_{v'}(X)] -
\E[b\phi_{v'}(Y)]\right| =\left|\E[\phi_{v'}(X)] - \E[\phi_{v'}(Y)]\right|.
\]
To prove this claim, write $v \in [-1/2,1/2]^n$ as $v = v' + w$ for $v \in [-1/4,1/4]^n$ and $w \in
\{-1/2,1/2\}^n$. Hence we have $\phi_v(x) = \phi_{v'}(x)\phi_w(x)$.
But for $x \in \pmo^n$,  $\sum_{i=1}^nw_ix_i \in \Z$ if $n$ is even, so that
$\phi_w(x) =1$ or $\sum_{i=1}^nw_ix_i -1/2 \in \Z$  if $n$ is odd, in which
case $\phi_w(x)  = -1$.

We round each coordinate $v_i$ to the nearest multiple of
$1/\lceil n/\delta\rceil$, so that it can be represented with $O(\log(n/\delta))$ bits
of precision. It is easy to see that for any $x \in \pmo^n$ this changes $\sum_iv_ix_i$ by at
most $\delta$, and $\phi_v(x)$ by at most $O(\delta)$. Hence, the
rounding only changes $\E[\phi_v(X)$ and $\E[\phi_v(Y)]$ by $O(\delta)$.
\end{proof}


Given this lemma, in our proofs, we only consider vectors $v$ which satsify the
conditions in Lemma \ref{lem:bounded} to error $\delta$. The same
generator then fools all $v$ with error $O(\delta)$, which
we will henceforth  ignore. One advatange of $v$ having bounded precision is
that we can compute $\phi_v$ using a small ROBP, the slight subtlelty
is that $\phi_v$ is a complex valued function and ROBPs can only
compute Boolean functions. We get around this by considering $g\circ
\phi_v$ for arbitrary functions $g:\C \rgta \pmo$. The ROBP for $g \circ
\phi_v$ keeps track of the sum $\sum_{j \leq k}v_jx_j$ for $1 \leq k
\leq n$ using $O(\log(n/\delta))$ bits of
precision. We label the states at layer $n$ with $-1$ or $1$ according
to $g$.

\begin{lem}
Let $v \in [1/4,1/4]^n$ have $O(\log(n/\delta))$ bits of precision. For
any $g:\C \rgta \pmo$, $g\circ \phi_v:\pmo^n \rgta \pmo$ can be
computed by an $(O(\log(n/\delta),1,n)$-ROBP.
\end{lem}



A corollary is that one can fool $\E[\phi_v]$ using $\prg$s for
bounded space. This will be useful once we reduce the dimension to $n'= O(\log^c(n))$.

\begin{cor}\label{smallnGenerator}
For $n',\delta>0$, there exists an explicit $\prg$ $\calG^{INW}:\zo^r \to \dpm^{n'}$
with seed-length $O(\log(n')\log(n'/\delta))$ so that for $X\in_u\{\pm
1\}^{n'}$, $z \in_u \zo^r$ and $v\in \R^n$
\[
\left|\E[\phi_v(X)] - \E[\phi_v(\calG(z))] \right| \leq O(\delta).
\]
\end{cor}
\begin{proof}
It suffices to consider $v$s with bounded precision.
Let $\calG^{INW}$ be the generator from Theorem \ref{th:inwprg} with seed length
\[ O(\log(n'/\delta)+\log(n')\log(4n'/\delta)) = O(\log(n')\log(n'/\delta)).\]
Since $\calG$ fools $g\circ \phi_v$ for all $g: \C \rgta \pmo$, we
have that $d_{TV}(\phi_v(X),\phi_v(Y)) \leq \delta/4$.  Since
$|\phi_v(X)| \leq 1$ and similarly for $\phi_v(Y)$, their expectations
differ by at most $\delta/2$.
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

